On the stability of the Bresse system with frictional damping

In this paper, we consider the Bresse system with frictional damping terms and prove some optimal decay results for the $L^2$-norm of the solution and its higher order derivatives. In fact, if we consider just one damping term acting on the second equation of the solution, we show that the solution does not decay at all. On the other hand, by considering one damping term alone acting on the third equation, we show that this damping term is strong enough to stabilize the whole system. In this case, we found a completely new stability number that depends on the parameters in the system. In addition, we prove the optimality of the results by using eigenvalues expansions. Our obtained results have been proved under some assumptions on the wave speeds of the three equations in the Bresse system.

==> esint.tex <==
% esint.tex 1.0 2005/06/21 -- macros for esint integral font
%%%@TeX-definition-file {
%%% filename       = "esint.tex",
%%% version        = "1.0",
%%% date           = "2005/06/21",
%%% package        = "esint 1.0",
%%% author         = "Michael M. Tung",
%%% email          = "mtung@mat.upv.es",
%%% address        = "Universidad Politécnica de Valencia,
%%%                   Departamento de Matemática Aplicada,
%%%                   Camino de Vera, s/n,
%%%                   46022 Valencia (Spain)",
%%% codetable      = "USASCII",
%%% keywords       = "TeX, plain TeX, style file",
%%% supported      = "Maybe",
%%% abstract       = "plain TeX macro to use the esint integral
%%%                   symbols available at CTAN or the website
%%%                   http://perso.wanadoo.fr/eddie.saudrais",
%%% copyright      = "Copyright (c) 2005 Michael M. Tung",
%%% copying        = "DISTRIBUTE THIS FILE AS YOU WISH.",
%%% dependencies   = "esint10.pfb,esint10.tfm".
%%%}

\message{1.0 <esint 2005/06/21}

\font\esint=esint10 

\def\int{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char02\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char01\kern1pt}}}{}{}}
\def\iint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char04\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char03\kern1pt}}}{}{}}
\def\iiint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char06\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char05\kern1pt}}}{}{}}
\def\iiiint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char08\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char07\kern1pt}}}{}{}}
\def\dotsint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char10\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char09\kern1pt}}}{}{}}
\def\oint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char12\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char11\kern1pt}}}{}{}}
\def\oiint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char14\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char13\kern1pt}}}{}{}}
\def\varoiint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char34\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char33\kern1pt}}}{}{}}
\def\sqint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char16\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char15\kern1pt}}}{}{}}
\def\sqiint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char18\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char17\kern1pt}}}{}{}}
\def\ointclockwise{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char24\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char23\kern1pt}}}{}{}}
\def\ointctrclockwise{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char26\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char25\kern1pt}}}{}{}}
\def\varointclockwise{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char28\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char27\kern1pt}}}{}{}}
\def\varointctrclockwise{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char30\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char29\kern1pt}}}{}{}}
\def\fint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char32\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char31\kern1pt}}}{}{}}
\def\landupint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char36\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char35\kern1pt}}}{}{}}
\def\landdownint{\mathchoice
{\mathop{\raise14pt\hbox{\esint\char38\kern4pt}}}
{\mathop{\raise8pt\hbox{\esint\char37\kern1pt}}}{}{}}

%
% end of file esint.tex
%

